Action Scene Graphs for Long-Form Understanding of Egocentric Videos

We present Egocentric Action Scene Graphs (EASGs), a new representation for long-form understanding of egocentric videos. EASGs extend standard manually-annotated representations of egocentric videos, such as verb-noun action labels, by providing a temporally evolving graph-based description of the actions performed by the camera wearer, including interacted objects, their relationships, and how actions unfold in time. Through a novel annotation procedure, we extend the Ego4D dataset by adding manually labeled Egocentric Action Scene Graphs offering a rich set of annotations designed for long-from egocentric video understanding. We hence define the EASG generation task and provide a baseline approach, establishing preliminary benchmarks. Experiments on two downstream tasks, egocentric action anticipation and egocentric activity summarization, highlight the effectiveness of EASGs for long-form egocentric video understanding. We will release the dataset and the code to replicate experiments and annotations.

==> sec/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Graph representations have emerged as a tool to encapsulate complex relationships and interactions in visual data, offering a structured pathway to encode visual scenes \cite{wu2021towards,ji2020action}. 
The ability to distill high-dimensional visual information into graph structures paves the way for an array of applications, significantly easing the challenge of interpreting and analyzing visual data. Graph representations have helped to advance a multitude of vision tasks, notably in areas such as image captioning \cite{nguyen2021defense,yang2019auto}, retrieval \cite{johnson2015image,patel2021multi,schroeder2020structured} and Visual Question Answering (VQA) \cite{mao2022dynamic,zhang2019empirical} among others. By leveraging the expressive power of graphs, these tasks have benefited from enriched contextual representations and improved performance in capturing intricate visual relationships and semantics. 
One of the current challenges of computer vision is the long-form understanding of videos, which entails decoding the evolving dynamics over extended time frames. This challenge is particularly relevant in eogocentric vision, where the interactions between humans and objects naturally unfold over time.

Egocentric vision can be useful for applications sprawling across fields such as robotics and augmented reality \cite{plizzari2023outlook, rodin2021predicting}, where human-object interactions play a central role in video understanding. Egocentric vision, capturing the visual perspective of a person interacting with objects in their environment, unfolds a unique canvas to study these interactions intimately. In this paper, we propose a novel approach to encoding egocentric human-object interactions in the form of scene graphs, which meticulously capture the relationships between the camera wearer and manipulated objects. We showcase that egocentric action scene graph representations are beneficial for downstream tasks related to long-form activity understanding from egocentric videos, thereby addressing the aforementioned challenge of long-form video understanding.

We build on the Ego4D dataset \cite{grauman2022ego4d}, which provides egocentric videos of individuals engaged in everyday activities. We annotate a subset of Ego4D videos with action scene graphs, encoding not only the objects partaking in the activities but also the relationships between these objects and the camera wearer. These annotated scene graphs serve as a robust benchmark for downstream tasks of egocentric action anticipation and long-form activity summarization.

We benchmark the scene graph generation task, mostly adapting models from existing works on scene graph generation \cite{li2022sgtr,feng2023exploiting,nag2023unbiased} and we tailor these models for the downstream tasks that leverage generated action scene graphs. Our endeavor underscores the potential of scene graphs in encoding human-object interactions within egocentric vision, offering a promising direction for future research in this field.
